Anthropogenic Mixing of Seasonally Stratified Shelf Seas by Offshore Wind Farm Infrastructure

The offshore wind energy sector has rapidly expanded over the past two decades, providing a renewable energy solution for coastal nations. Sector development has been led in Europe, but is growing globally. Most developments to date have been in well-mixed, i.e. unstratified, shallow-waters near to shore. Sector growth is, for the first time, pushing developments to deep water, into a brand new environment: seasonally stratified shelf seas. Seasonally stratified shelf seas, where water density varies with depth, have a disproportionately key role in primary production, marine ecosystem and biochemically cycles. Infrastructure will directly mix stratified shelf seas. The magnitude of this mixing, additional to natural background processes, has yet to be fully quantified. If large enough it may erode shelf sea stratification. Therefore, offshore wind growth may destabilize and fundamentally change shelf sea systems. However, enhanced mixing may also positively impact some marine ecosystems. This paper sets the scene for sector development into this new environment, reviews the potential physical and environmental benefits and impacts of large scale industrialization of seasonally stratified shelf seas and identifies areas where research is required to best utilise, manage and mitigate environmental change.

==> Figures_Final/figure_permissions.tex <==
JFM publications: The first Figure/Table can be reused at no charge on the understanding that it is not acknowledged to another source. Cambridge University Press grants a license for all orders, including \$0 orders. Please select the Continue button and place an order for this reuse.

Figure 1A   Original Image
Figure 1B   Original Image
Figure 1C   This is an open access article under the terms of the Creative Commons Attribution License, which permits use, distribution and reproduction in any medium, provided the original work is properly cited. https://abdn.pure.elsevier.com/en/publications/fishing-and-the-oceanography-of-a-stratified-shelf-sea

Figure 2    Original Image

Figure 3    Original Image

Figure 4    Open access publication Copyright © 2013 The Author (J. Sharples). Published by Elsevier Ltd. Open access under CC BY license.  https://abdn.pure.elsevier.com/en/publications/from-physics-to-fishing-over-a-shelf-sea-bank

Figure 5    Open access under CC BY license

Figure 6    Original Image

Figure 7    Charlie

Figure 8    Original Image

Figure 9a   See 9b, and we have permissions from author.

Figure 9b   Crown estate copywrite: (Is our reference fine here?)  
This publication (excluding the logos) may be re-used free of  
charge in any format or medium. It may only be used accurately and 
not in a misleading context. The material must be acknowledged as The Crown Estate copyright and use of it must give the title of the source publication. Where third party copyright material has been identified, further use of that material requires permission from the copyright holders concerned.


Figure 10A  JFM Publication
Figure 10B  JFM Publication

Figure 11   JFM Publication

Figure 12   Charlie to email authors, publication is open access:
This is an open access article under the terms of the Creative Commons Attribution License, which permits use, distribution and reproduction in any medium, provided the original work is properly cited.

Figure 13   Original Image

Figure 14   Original Image
